Densities of Almost Surely Terminating Probabilistic Programs are Differentiable Almost Everywhere

We study the differential properties of higher-order statistical probabilistic programs with recursion and conditioning. Our starting point is an open problem posed by Hongseok Yang: what class of statistical probabilistic programs have densities that are differentiable almost everywhere? To formalise the problem, we consider Statistical PCF (SPCF), an extension of call-by-value PCF with real numbers, and constructs for sampling and conditioning. We give SPCF a sampling-style operational semantics a la Borgstrom et al., and study the associated weight (commonly referred to as the density) function and value function on the set of possible execution traces. Our main result is that almost-surely terminating SPCF programs, generated from a set of primitive functions (e.g. the set of analytic functions) satisfying mild closure properties, have weight and value functions that are almost-everywhere differentiable. We use a stochastic form of symbolic execution to reason about almost-everywhere differentiability. A by-product of this work is that almost-surely terminating deterministic (S)PCF programs with real parameters denote functions that are almost-everywhere differentiable. Our result is of practical interest, as almost-everywhere differentiability of the density function is required to hold for the correctness of major gradient-based inference algorithms.

==> notes.tex <==
% !TEX root = ./main-repara.tex
\renewcommand{\charfn}[1]{\mathbbl{1}[#1]}

[Note 21 April 2020]

\paragraph*{Possible directions}

\begin{enumerate} 
\item We could extend \cite{DBLP:conf/nips/0001YY18} in the same style, i.e., abstract treatment in terms of joint distribution $p(\tupf x, \tupf z)$ and variational distribution $q_\theta(\tupf z)$ (without reference to the probabilistic programs defining the distributions); 
followed by an empirical study.

\item A related project is to study the extended algorithm from a verification angle, in the style as \cite{DBLP:journals/pacmpl/LeeYRY20}, i.e., develop methods to verify the correctness / convergence conditions.
\end{enumerate}

\section{Extending VI reparametrisation gradient algorithm \cite{DBLP:conf/nips/0001YY18} to unbounded models}


\paragraph*{\cite[Theorem 1]{DBLP:conf/nips/0001YY18}}

\cite[Theorem 1]{DBLP:conf/nips/0001YY18} seems to extend as desired.

- We assume that the vector of latent variables $\tupf z$ ranges over the trace space $\traces$.

- The variational distribution $q_\theta(\tupf z)$ is parameterised by, and continuously differentiable w.r.t., $\theta \in \Real^d$, as in \cite{DBLP:conf/nips/0001YY18}.

- Moreover $q_\theta(z)$ is the distribution of $z = f_\theta(\tupf \epsilon)$ for a smooth function $f : \Real^d \times \traces \to \traces$ and a random variable $\tupf \epsilon \in \traces$ distributed by density $q(\tupf \epsilon) = q_\theta(f_\theta(\tupf \epsilon)) \cdot |\textrm{det} \, \nabla_{\tupf \epsilon} \, f_\theta(\tupf \epsilon)|$, and $q(\tupf \epsilon)$ is required to be independent of $\theta$.

- Further $f_\theta$ is bijective on $\traces$; and the image of ${f_\theta \mid_{\Real^m}{}} : \Real^m \to \traces$ is $\Real^m$ (and so, bijective on $\Real^m$), for each $\theta \in \Real^d$.

- We assume that the joint density $r(\tupf z) = p({\tupf x}_0, \tupf z)$ at $\tupf x = {\tupf x}_0$ is piecewise (continuously) differentiable, i.e., has the form
\[
r(\tupf z) = \sum_{i \in \Nat} \sum_{j \in \Nat} \charfn{{\tupf z} \in R_{ij}} \cdot r_{ij} (\tupf z)
\] 
where for each $i \in \Nat$
\begin{itemize}
\item $\{R_{ij}\}_{j \in \Nat}$ is a smooth partition of $\Real^i$, and $\leb_i(\boundary R_{ij}) = 0$

\item for each $j \in \Nat$, $r_{ij} : \Real^i \to \pReal$ is (continuously) differentiable.
\end{itemize}

- Usual hygiene conditions: absolute continuity, and integrability of the ELBO integral.

- Assumptions on $q_\theta$: What forms do they take? Ideally we would want them to have the same control structure as the programs they approximate (and so, definable using conditionals, and even recursion).

\subparagraph{Examples of reparameterisation} 1D Gaussian: $q_\theta(z)$ is the density for Gaussian with mean $\mu$ and variance $\sigma^2$, and $q(\epsilon)$ is the density for the standard normal, with $f_\theta(\epsilon) = \sigma \cdot \epsilon + \mu$. 

- Factorised Gaussian: $q_\theta(\tupf z) = \mathcal{N}(\tupf z; \tupf \mu, \textrm{diag}({\tupf \sigma}^2))$. I.e.~
\[
q_\theta(\tupf z) = \prod_i q_\theta(z_i) = \prod_i \mathcal{N}(z_i; \mu_i, \sigma_i^2)
\]
After reparameterisation, we have $\epsilon \sim \mathcal{N}(0, \mathbf I)$ with $\tupf z = f_\theta(\tupf \epsilon) = \tupf \mu + \tupf \sigma \odot \tupf \epsilon$ (where $\odot$ is element-wise product).

- Full covariance Gaussian (Cholesky): $q_\theta(\tupf z) = \mathcal{N}(\tupf z; \tupf \mu, \mathbf \Sigma)$. After reparameterisation, we have $\epsilon \sim \mathcal{N}(0, \mathbf I)$ with $\tupf z = f_\theta(\tupf \epsilon) = \tupf \mu + {\mathbf L} \, \tupf \epsilon$ where $\mathbf L$ is chosen to be a upper (or lower) triangular matrix with non-zero diagonal elements.
N.B.~Jacobian is easy $\frac{\partial \tupf z}{\partial \tupf \epsilon} = \mathbf L$: conveniently the determinant of a triangular matrix is the product of its diagonals.
This corresponds to the Cholesky decomposition $\mathbf \Sigma = \mathbf L \, {\mathbf L}^T$ of the covariance of $\tupf z$ (see \cite{DBLP:journals/ftml/KingmaW19}).


\paragraph*{Limitations of reparametrisation gradients} 
The requirement that the transformed density $q(\tupf \epsilon)$ be independent of the variational parameter $\theta$ is constraining.
The reparameterisation gradient algorithm works well for the Gaussian distribution, but not for (the widely used) Beta and Gamma distributions.
In their original treatment of reparameterisation gradients, Kingma and Welling \cite{DBLP:journals/corr/KingmaW13} discuss three families of transforms: inverse cummulative density function, location-scale, and composition. 
However they do not apply in certain cases (see \cite{DBLP:conf/nips/RuizTB16}).

\emph{Generalized reparameterizations} \cite{DBLP:conf/nips/RuizTB16} use invertible transformations of the latent variables, which lead to transformed distributions that \emph{weakly} depend (i.e.~at least its first moment does not depend) on the variational parameters. 
This results in new Monte Carlo gradients that combine reparameterization gradients and score function gradients. 
The generalized reparameterization is effective (even a single sample from the variational distribution is enough to obtain a low-variance gradient), and it works on nonconjugate models, using variational approximations involving beta and gamma distributions.

\paragraph*{\cite[Theorem 6]{DBLP:conf/nips/0001YY18}}

- In order to apply Theorem 6 to Theorem 1, we need $\theta$ to range over $\Real^d$ (as opposed to $\Real$).

- A key step in Theorem 1 (i.e.~(7) in Appendix A) involves ``differentiating under the integral sign'', which is supposed to be justified by Theorem 6. 
Here the ``differentiation'' takes the form of gradient w.r.t.~the variational parameter $\theta$, which ranges over $\Real^d$. 
However, the $\theta$ in Theorem 6 ranges over $\Real$: it is intuitively the dimension of time, following (4.1) of \cite{Flanders73} which is used to justify Theorem 6.

What the authors of \cite{DBLP:conf/nips/0001YY18} tacitly assume is that Theorem 6 generalises to gradient in $d$-dimensional space. 
Theorem 6 is quite standard in fluid dynamics, and is called Reynolds Transport Theorem. 
There is a detailed discussion of the Theorem in \cite[p.~22]{Leal07}, stressing the physical intuition, and a proof.

\paragraph*{Estimating the surface integral}

\section{Inference on unbounded models: examples}

\subsection{Mixture model with a random number of clusters}

We say that the \emph{address-trace} of a run of a program is the sequence of the addresses of the encountered sample commands.

A program is said to have \emph{stochastic support} if the address-trace varies between runs.

Here is a (non-trivial and possibly challenging) test problem involving a program with stochastic support. 

A simple 1D Gaussian mixture model with a random number of clusters $K$ (sampled from a Poisson distribution).
\begin{align*}
K &\sim \textrm{Poisson}(9) + 1\\
\mu_k &\sim \textrm{Uniform}\Big(\frac{20(k-1)}{K}, \frac{20k}{K}\Big)\\
z_n &\sim \textrm{Cat}\Big(\frac{1}{K}, \ldots, \frac{1}{K}\Big)\\
y_n &\sim \textrm{N}(\mu_{z_n}, 0.1^2)\\
\end{align*}
Using the model, generate a synthetic dataset of $y_{1:150}$ for a mixture of $K=5$ clusters.

Perform inference on $K$ and $\mu_{1:K}$.

\emph{This is not a simple problem for probabilistic programming (to provide generic inference)}: ``In fact, we are not aware of any fully automated inference engine that is able to give satisfactory performance, despite the apparent simplicity of the problem.'' \cite{DBLP:journals/corr/abs-1910-13324}

\subsection{Bayesian nonparametric models}




==> out <==
This is pdfTeX, Version 3.14159265-2.6-1.40.19 (TeX Live 2018) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2018-04-01> patch level 2
Babel <3.18> and hyphenation patterns for 84 language(s) loaded.
(./llncs.cls
Document Class: llncs 2018/03/10 v2.20 
 LaTeX document class for Lecture Notes in Computer Science
(/usr/local/texlive/2018/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2018/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2018/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/aliascnt.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/carlisle/remreset.sty)))
(./preamble.tex (/usr/local/texlive/2018/texmf-dist/tex/latex/amscls/amsthm.sty
) (./commenting.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics-def/pdftex.def))
(/usr/local/texlive/2018/texmf-dist/tex/latex/bbding/bbding.sty))
(/usr/local/texlive/2018/texmf-dist/tex/generic/ulem/ulem.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2018/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2018/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2018/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2018/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/jknapltx/mathbbol.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/etex-pkg/etex.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/stmaryrd/stmaryrd.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/mathtools/mhsetup.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsmath/amsopn.sty)

Package amsmath Warning: Unable to redefine math accent \vec.

)) (/usr/local/texlive/2018/texmf-dist/tex/latex/doublestroke/dsfont.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/relsize/relsize.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/bussproofs/bussproofs.sty
Proof Tree (bussproofs) style macros. Version 1.1.
) (/usr/local/texlive/2018/texmf-dist/tex/latex/lkproof/proof.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/listings.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/local/texlive/2018/texmf-dist/tex/latex/tools/tabularx.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/tools/array.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/tabulary/tabulary.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xy.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xy.tex Bootstrap'ing:
catcodes, docmode,
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyrecat.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyidioms.tex)

 Xy-pic version 3.8.9 <2013/10/06>
 Copyright (c) 1991-2013 by Kristoffer H. Rose <krisrose@tug.org> and others
 Xy-pic is free software: see the User's Guide for details.

Loading kernel: messages; fonts; allocations: state, direction,
utility macros; pictures: \xy, positions, objects, decorations;
kernel objects: directionals, circles, text; options; algorithms: directions,
edges, connections;  Xy-pic loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyall.tex
 Xy-pic option: All features v.3.8
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xycurve.tex
 Xy-pic option: Curve and Spline extension v.3.12 curve, circles, loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyframe.tex
 Xy-pic option: Frame and Bracket extension v.3.14 loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xycmtip.tex
 Xy-pic option: Computer Modern tip extension v.3.7
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xytips.tex
 Xy-pic option: More Tips extension v.3.11 loaded) loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyline.tex
 Xy-pic option: Line styles extension v.3.10 loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyrotate.tex
 Xy-pic option: Rotate and Scale extension v.3.8 loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xycolor.tex
 Xy-pic option: Colour extension v.3.11 loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xymatrix.tex
 Xy-pic option: Matrix feature v.3.14 loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xyarrow.tex
 Xy-pic option: Arrow and Path feature v.3.9 path, \ar, loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xygraph.tex
 Xy-pic option: Graph feature v.3.11 loaded) loaded)
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf.tex
 Xy-pic option: PDF driver v.1.7 Xy-pic pdf driver: `color' extension support
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf-co.tex loaded)
Xy-pic pdf driver: `curve' extension support
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf-cu.tex loaded)
Xy-pic pdf driver: `frame' extension support
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf-fr.tex loaded)
Xy-pic pdf driver: `line' extension support
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf-li.tex loaded)
Xy-pic pdf driver: `rotate' extension support
(/usr/local/texlive/2018/texmf-dist/tex/generic/xypic/xypdf-ro.tex loaded)
loaded))
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-li
sts.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
(/usr/local/texlive/2018/texmf-dist/tex/latex/ms/everyshi.sty))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.c
ode.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex)
) (/usr/local/texlive/2018/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.cod
e.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothan
dlers.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.cod
e.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytopaths.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unsupported document class (or package) detected,
(caption)                usage of the caption package is not recommended.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2018/texmf-dist/tex/latex/ifsym/ifsym.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/lstlang1.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/lstlang2.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2018/texmf-dist/tex/generic/tikz-cd/tikzlibrarycd.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarymatrix.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryquotes.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.
meta.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytrees.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.geometric.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.geometric.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.misc.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.misc.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.symbols.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.symbols.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.arrows.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.arrows.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.callouts.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.callouts.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.multipart.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.multipart.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarypatterns.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/pgflibrarypattern
s.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/latex/cleveref/cleveref.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-restate.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thmtools.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-patch.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/parseargs.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-kv.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-autoref.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/aliasctr.sty))
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-listof.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-amsthm.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/thmtools/thm-llncs.sty

Package thmtools Warning: LLNCS support disables automatic casing of theorem na
mes .

))) (/usr/local/texlive/2018/texmf-dist/tex/latex/filecontents/filecontents.sty
) (/usr/local/texlive/2018/texmf-dist/tex/latex/pgfplots/pgfplots.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.revision.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotscore.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/sys/pgfplotssysgeneric
.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/libs/pgfplotslibrary.c
ode.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_loader.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/pgflibraryfpu.cod
e.tex)
Package pgfplots: loading complementary arithmetics for your pgf version...

(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_pgflibraryfpu.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_pgfmathfloat.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_leq.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotsutil.code
.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
liststructure.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
liststructureext.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
array.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
matrix.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/numtable/pgfplotstable
shared.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
deque.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotsbinary.co
de.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotsbinary.da
ta.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotsutil.verb
.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/libs/pgflibrarypgfplot
s.surfshading.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/sys/pgflibrarypgfplots
.surfshading.pgfsys-pdftex.def)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotscolormap.
code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/util/pgfplotscolor.cod
e.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotsstackedplots.c
ode.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotsplothandlers.c
ode.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotsmeshplothandle
r.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotsmeshplotimage.
code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.scaling.code.
tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotscoordprocessin
g.code.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.errorbars.cod
e.tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.markers.code.
tex)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplotsticks.code.tex
)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.paths.code.te
x)
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/modules/pgfmoduledecoration
s.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathmorphing.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathmorphing.code.tex))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathreplacing.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathreplacing.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryplotmarks.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgf/libraries/pgflibraryplotmar
ks.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/latex/pgfplots/pgfplotstable.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/pgfplots.revision.tex)

(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/numtable/pgfplotstable
.code.tex
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/numtable/pgfplotstable
.coltype.code.tex)))
(/usr/local/texlive/2018/texmf-dist/tex/generic/pgfplots/libs/tikzlibrarypgfplo
ts.statistics.code.tex)) (./macros.tex) (./main.aux)
(/usr/local/texlive/2018/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2018/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2018/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2018/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2018/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./main.out) (./main.out)
(/usr/local/texlive/2018/texmf-dist/tex/latex/bbold/Ubbold.fd)
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2018/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2018/texmf-dist/tex/latex/stmaryrd/Ustmry.fd)
ABD: EveryShipout initializing macros
Package pgfplots notification 'compat/show suggested version=true': document ha
s been generated with the most recent feature set (\pgfplotsset{compat=1.16}).

(/usr/local/texlive/2018/texmf-dist/tex/latex/ifsym/uifsym.fd)

LaTeX Font Warning: Font shape `OMS/cmtt/m/n' undefined
(Font)              using `OMS/cmsy/m/n' instead
(Font)              for symbol `textbraceleft' on input line 78.

(./introduction.tex [1{/usr/local/texlive/2018/texmf-var/fonts/map/pdftex/updma
p/pdftex.map} <./orcid_color-eps-converted-to.pdf>] [2]) (./probprog.tex
[3] (/usr/local/texlive/2018/texmf-dist/tex/latex/base/omscmr.fd)
(/usr/local/texlive/2018/texmf-dist/tex/latex/base/omlcmr.fd) [4] [5])
(./semantics.tex [6]

LaTeX Font Warning: Font shape `U/stmry/b/n' undefined
(Font)              using `U/stmry/m/n' instead on input line 65.

[7] [8] [9]) (./diff.tex [10] [11] [12] [13] [14]) (./symbolic.tex [15]
(/usr/local/texlive/2018/texmf-dist/tex/latex/psnfss/ot1pzc.fd)
Overfull \hbox (28.08395pt too wide) detected at line 312
[]
[16] [17] [18]

LaTeX Font Warning: Font shape `OT1/cmss/m/it' in size <10> not available
(Font)              Font shape `OT1/cmss/m/sl' tried instead on input line 559.


[19] [20]) (./termdiff.tex [21] [22] [23]) (./conclusion.tex [24]) (./main.bbl
[25] [26] [27] [28] [29]) [30 <./cc_by_4-0-eps-converted-to.pdf>] (./main.aux)

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(\end occurred inside a group at level 1)

### simple group (level 1) entered at line 62 ({)
### bottom level
(\end occurred when \iftrue on line 149 was incomplete)
(\end occurred when \iftrue on line 26 was incomplete)
(\end occurred when \iftrue on line 25 was incomplete)
(\end occurred when \iftrue on line 106 was incomplete)
(\end occurred when \iftrue on line 769 was incomplete)
(\end occurred when \iftrue on line 637 was incomplete)
(\end occurred when \iftrue on line 632 was incomplete)
(\end occurred when \iftrue on line 559 was incomplete)
(\end occurred when \iftrue on line 539 was incomplete)
(\end occurred when \iftrue on line 478 was incomplete)
(\end occurred when \iftrue on line 478 was incomplete)
(\end occurred when \iftrue on line 454 was incomplete)
(\end occurred when \iftrue on line 432 was incomplete)
(\end occurred when \iftrue on line 429 was incomplete)
(\end occurred when \iftrue on line 285 was incomplete)
(\end occurred when \iftrue on line 512 was incomplete)
(\end occurred when \iftrue on line 436 was incomplete)
(\end occurred when \iftrue on line 423 was incomplete)
(\end occurred when \iftrue on line 372 was incomplete)
(\end occurred when \iftrue on line 367 was incomplete)
(\end occurred when \iftrue on line 57 was incomplete)
(\end occurred when \iftrue on line 50 was incomplete)
(\end occurred when \iftrue on line 46 was incomplete)
(\end occurred when \iftrue on line 34 was incomplete)
(\end occurred when \iftrue on line 33 was incomplete)
(\end occurred when \iftrue on line 27 was incomplete)
(\end occurred when \iftrue on line 15 was incomplete)
(\end occurred when \iftrue on line 11 was incomplete)
(\end occurred when \iftrue on line 416 was incomplete)
(\end occurred when \iftrue on line 95 was incomplete)
(\end occurred when \iftrue on line 206 was incomplete)
(\end occurred when \iftrue on line 203 was incomplete)
(\end occurred when \iftrue on line 193 was incomplete)
(\end occurred when \iftrue on line 192 was incomplete)
(\end occurred when \iftrue on line 186 was incomplete)
(\end occurred when \iftrue on line 14 was incomplete)
(\end occurred when \ifmmode on line 7 was incomplete)
(\end occurred when \iftrue on line 70 was incomplete)
(\end occurred when \iftrue on line 69 was incomplete)
(\end occurred when \iftrue on line 42 was incomplete)
(\end occurred when \iftrue on line 19 was incomplete)
(\end occurred when \iftrue on line 5 was incomplete)
(see the transcript file for additional information){/usr/local/texlive/2018/te
xmf-dist/fonts/enc/dvips/mnsymbol/MnSymbolE.enc}{/usr/local/texlive/2018/texmf-
dist/fonts/enc/dvips/base/8r.enc} </Users/domner/Library/texlive/2018/texmf-var
/fonts/pk/ljfour/public/ifsym/ifsym10.420pk></usr/local/texlive/2018/texmf-dist
/fonts/type1/public/mnsymbol/MnSymbol10.pfb></usr/local/texlive/2018/texmf-dist
/fonts/type1/public/mnsymbol/MnSymbol7.pfb></usr/local/texlive/2018/texmf-dist/
fonts/type1/public/mnsymbol/MnSymbol9.pfb></usr/local/texlive/2018/texmf-dist/f
onts/type1/public/bbold-type1/bbold10.pfb></usr/local/texlive/2018/texmf-dist/f
onts/type1/public/bbold-type1/bbold7.pfb></usr/local/texlive/2018/texmf-dist/fo
nts/type1/public/amsfonts/cmextra/cmbsy7.pfb></usr/local/texlive/2018/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2018/texmf-dist
/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/local/texlive/2018/texmf-dist/
fonts/type1/public/amsfonts/cm/cmbx9.pfb></usr/local/texlive/2018/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmbxti10.pfb></usr/local/texlive/2018/texmf-dist/f
onts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2018/texmf-dist/fo
nts/type1/public/amsfonts/cmextra/cmex7.pfb></usr/local/texlive/2018/texmf-dist
/fonts/type1/public/amsfonts/cmextra/cmex9.pfb></usr/local/texlive/2018/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2018/texmf-di
st/fonts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2018/texmf-dist
/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2018/texmf-dist/f
onts/type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2018/texmf-dist/fon
ts/type1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2018/texmf-dist/fonts
/type1/public/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2018/texmf-dist/fonts
/type1/public/amsfonts/cmextra/cmmib9.pfb></usr/local/texlive/2018/texmf-dist/f
onts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2018/texmf-dist/fon
ts/type1/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2018/texmf-dist/fonts/
type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2018/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr7.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/
public/amsfonts/cm/cmr9.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmss10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/publ
ic/amsfonts/cm/cmss8.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public
/amsfonts/cm/cmss9.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/a
msfonts/cm/cmssi10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/am
sfonts/cm/cmsy5.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy6.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmsy7.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy9.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfonts/c
m/cmti10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfonts/cm
/cmti9.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfonts/cm/c
mtt9.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/amsfonts/symbol
s/msbm10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/stmaryrd/st
mary10.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/public/stmaryrd/stma
ry7.pfb></usr/local/texlive/2018/texmf-dist/fonts/type1/urw/zapfchan/uzcmi8a.pf
b>
Output written on main.pdf (30 pages, 557795 bytes).
Transcript written on main.log.

